Width Provably Matters in Optimization for Deep Linear Neural Networks

We prove that for an $L$-layer fully-connected linear neural network, if the width of every hidden layer is $\tilde\Omega (L \cdot r \cdot d_{\mathrm{out}} \cdot \kappa^3 )$, where $r$ and $\kappa$ are the rank and the condition number of the input data, and $d_{\mathrm{out}}$ is the output dimension, then gradient descent with Gaussian random initialization converges to a global minimum at a linear rate. The number of iterations to find an $\epsilon$-suboptimal solution is $O(\kappa \log(\frac{1}{\epsilon}))$. Our polynomial upper bound on the total running time for wide deep linear networks and the $\exp\left(\Omega\left(L\right)\right)$ lower bound for narrow deep linear neural networks [Shamir, 2018] together demonstrate that wide layers are necessary for optimizing deep models.

==> stuff.tex <==





%\section{Small perturbations do not affect properties at initialization}
%
%\begin{lem}
%	Suppose weight matrices $W_1, \ldots, W_L$ satisfy 
%	$\norm{W_k - W_k(0)} \le \Delta$ $(\forall k\in[L])$.
%	Then for any $1< i \le j < L$ we have \wei{assuming good init}
%	\begin{align*}
%	\norm{W_{j:i} - W_{j:i}(0)} \le something
%	\end{align*}
%\end{lem}
%\begin{proof}
%	Let $\Delta_k = W_k - W_k(0)$ for all $k$.
%	Then
%	\begin{align*}
%	W_{j:i} = \left( W_j(0) + \Delta_j \right) \cdots \left( W_i(0) + \Delta_i \right) .
%	\end{align*}
%	Each term except the leading term $W_{j:i}(0)$ has the form:
%	\begin{equation} \label{eqn:perturbation-terms}
%	\begin{aligned}
%	W_{j:(k_s+1)}(0)	\cdot \Delta_{k_s} \cdot W_{(k_s-1):(k_{s-1}+1)}(0) \cdot \Delta_{k_{s-1}} \cdots \\ \cdot \Delta_{k_1} \cdot W_{(k_1-1):i}(0)  ,
%	\end{aligned}
%	\end{equation}
%	where $i \le k_1 < \cdots < k_s \le j$ are positions at which perturbation terms $\Delta_{k_l}$ are taken out, and at any other position $k$, $W_k(0)$ is used.
%	Note that every factor in~\eqref{eqn:perturbation-terms} of the form $W_{b:a}(0)$ satisfies $\norm{W_{b:a}(0)} \le O\left(\sqrt Lm^{\frac{b-a+1}{2}}\right)$;
%	there are at most $s+1$ such factors, so the product of their spectral norms is at most $\left(O(\sqrt{L})\right)^{s+1} m^{\frac{j-i+1-s}{2}} $.
%	Thus, we can bound the sum of all perturbation terms as
%	\begin{align*}
%	&\norm{W_{j:i} - W_{j:i}(0)} \\
%	\le\,& \sum_{s=1}^{j-i+1} \binom{j-i+1}{s} \Delta^s \left( O\left(\sqrt L\right) \right)^{s+1} m^{\frac{j-i+1-s}{2}} \\
%	\le\,&  \sum_{s=1}^{j-i+1} L^t \Delta^s \left( O\left(\sqrt L\right) \right)^{s+1} m^{\frac{j-i+1-s}{2}} \\
%	=\,& O\left(\sqrt L\right) \sum_{s=1}^{j-i+1} \left( \frac{ O\left(L^{3/2}\Delta\right)}{\sqrt m} \right)^s   m^{\frac{j-i+1}{2}} \\
%	\le\,& c \sqrt{L} m^{\frac{j-i+1}{2}}
%	\end{align*}
%	for a small constant $c$ as long as $m > C L^3\Delta^2$ for a large constant $C$.
%\end{proof}
%\wei{for $i=1$ or $j=L$, we can drop the $\sqrt L$ factor}








\section{Error in discrete time}



\begin{align*}
W_{L:1}(t+1) - W_{L:1}(t) = \prod_i \left( W_i(t) - \eta \frac{\partial \ell}{\partial W_i}(t) \right) - W_{L:1}(t)\\
= -\eta \cdot something + E(t)
\end{align*}

Main equation:
\begin{align*}
&\vectorize{U(t+1) - U(t)} \\
=\,& -\eta P(t) \cdot \vectorize{U(t)-Y} + \frac{1}{\sqrt{m^{L-1}\dout}} \vectorize{E(t)X}
\end{align*}

$\eta \le  \frac{1}{\norm{P(t)}} = O\left( \frac{{\dout}}{L\norm{X}^2} \right)$

Bound $E(t)$
\begin{align*}
& \frac{1}{\sqrt{m^{L-1}\dout}} \norm{E(t) X}_F \\
\le\,& \frac{1}{\sqrt{m^{L-1}\dout}} \sum_{s=2}^L \binom{L}{s} \left(\eta \Delta(t) \right)^s \left( O\left(\sqrt L\right) \right)^{s-1} m^{\frac{L-s}{2}} \norm{X} \\
\le \,& \frac{1}{\sqrt{\dout}} \sum_{s=2}^L L^s \left(\eta \cdot O\left( \frac{\sqrt{\ell(t)}}{\sqrt{\dout}}  \right) \norm{X} \right)^s \left( O\left(\sqrt L\right) \right)^{s-1} m^{\frac{1-s}{2}} \norm{X} \\
= \,& \frac{1}{\sqrt{\dout}} \sum_{s=2}^L  \left(  O\left( \eta L^{3/2}\frac{\sqrt{\ell(t)}\norm{X}}{\sqrt{\dout}}  \right)  \right)^s  L^{-1} m^{\frac{1-s}{2}} \norm{X} \\
= \,& \frac{1}{\sqrt{\dout}} \sum_{s=2}^L  \left(  O\left( \eta L^{3/2}\frac{\sqrt{\ell(t)}\norm{X}}{\sqrt{m \dout}}  \right)  \right)^{s-1}  L^{-1}   \norm{X} \\ &\qquad \cdot \eta L^{3/2}\frac{\sqrt{\ell(t)}\norm{X}}{\sqrt{\dout}}  \\
= \,& \frac{\eta \sqrt{\ell(t)}\sqrt{L}   \norm{X}^2  }{\dout} \sum_{s=2}^L  \left(  O\left( \frac{\sqrt{\dout}}{L\norm{X}^2} L^{3/2}\frac{\sqrt{\ell(t)}\norm{X}}{\sqrt{m\dout}}  \right)  \right)^{s-1}   \\
= \,& \frac{\eta \sqrt{\ell(t)}\sqrt{L}   \norm{X}^2  }{\dout} \sum_{s=2}^L  \left(  O\left( \frac{\sqrt{L\cdot \ell(t)}}{\sqrt{m}\norm{X}}  \right)  \right)^{s-1}  
\end{align*}

We want this to be less than $\frac12 \eta \lambda_{\min}(P(t)) \norm{U(t)-Y}_F\ge \eta \Omega\left( \frac{L \sigma_{\min}^2(X)}{\dout} \right) \sqrt{\ell(t)}$

Need $m> C\frac{L\cdot \ell(t)}{\norm{X}^2}$ and
\begin{align*}
\frac{\eta \sqrt{\ell(t)}\sqrt{L}   \norm{X}^2  }{\dout} \frac{\sqrt{L\cdot \ell(t)}}{\sqrt{m}\norm{X}}  < c \eta  \frac{L \sigma_{\min}^2(X)}{\sqrt{\dout}} \sqrt{\ell(t)}
\end{align*}
which is
\begin{align*}
C \frac{   \norm{X}  }{} \frac{\sqrt{ \ell(t)}}{\sigma_{\min}^2(X)}  < \sqrt{m} 
\end{align*}
